Convergence of supercell and superspace methods for computing spectra of quasiperiodic operators

We study the convergence of two of the most widely used and intuitive approaches for computing the spectra of differential operators with quasiperiodic coefficients: the supercell method and the superspace method. In both cases, Floquet-Bloch theory for periodic operators can be used to compute approximations to the spectrum. We illustrate our results with examples of Schr\"odinger and Helmholtz operators.

==> Preamble.tex <==
\usepackage{graphicx} 
\usepackage{amssymb, amsmath}
\usepackage{geometry}
\usepackage{minted}
\usepackage{hyperref}             
\usepackage{subfig}
\numberwithin{equation}{section} 
\usepackage{mdframed}
\usepackage[table]{xcolor}
\usepackage[backend=biber,style=alphabetic]{biblatex}
\addbibresource{references.bib}         
\renewcommand{\baselinestretch}{1.04}        %line spacing
%\usepackage{afterpage}                      %emptypage
\usepackage[export]{adjustbox}

\hypersetup{
pdftitle={Convergence of supercell and superspace methods for computing spectra of quasiperiodic operators},
pdfsubject={quasicrystal, cut and project, fractal spectrum, Cantor set, Fibonacci tiling, almost Mathieu operator},
pdfauthor={BRYN DAVIES and CLEMENS THALHAMMER},
pdfkeywords={}
}

\newmdtheoremenv[backgroundcolor=green!0!white,linewidth=0pt,]{definition}{Definition}[section]
\newmdtheoremenv[backgroundcolor=yellow!0!white, linewidth=0pt,]{remark}{Remark}[section]
\newmdtheoremenv[backgroundcolor=yellow!0!white, linewidth=0.5pt,]{corollary}{Corollary}[section]
\newmdtheoremenv[backgroundcolor=red!0!white, linewidth=0.5pt,]{theorem}{Theorem}[section]
\newmdtheoremenv[backgroundcolor=red!0!white, linewidth=0.5pt,]{lemma}{Lemma}[section]
\newmdtheoremenv[backgroundcolor=white, linewidth=0pt,]{example}{Example}[section]

\newgeometry{inner = 3.5cm, outer = 3.5cm, top = 3.5cm, bottom = 3.5cm}
